SmartState: Detecting State-Reverting Vulnerabilities in Smart Contracts via Fine-Grained State-Dependency Analysis

Smart contracts written in Solidity are widely used in different blockchain platforms such as Ethereum, TRON and BNB Chain. One of the unique designs in Solidity smart contracts is its state-reverting mechanism for error handling and access control. Unfortunately, a number of recent security incidents showed that adversaries also utilize this mechanism to manipulate critical states of smart contracts, and hence, bring security consequences such as illegal profit-gain and Deny-of-Service (DoS). In this paper, we call such vulnerabilities as the State-reverting Vulnerability (SRV). Automatically identifying SRVs poses unique challenges, as it requires an in-depth analysis and understanding of the state-dependency relations in smart contracts. This paper presents SmartState, a new framework for detecting state-reverting vulnerability in Solidity smart contracts via fine-grained state-dependency analysis. SmartState integrates a set of novel mechanisms to ensure its effectiveness. Particularly, Smart-State extracts state dependencies from both contract bytecode and historical transactions. Both of them are critical for inferring dependencies related to SRVs. Further, SmartState models the generic patterns of SRVs (i.e., profit-gain and DoS) as SRV indicators, and hence effectively identify SRVs based on the constructed state-dependency graph. To evaluate SmartState, we manually annotated a ground-truth dataset which contains 91 SRVs in the real world. Evaluation results showed that SmartState achieves a precision of 87.23% and a recall of 89.13%. In addition, SmartState successfully identifies 406 new SRVs from 47,351 real-world smart contracts. 11 of these SRVs are from popular smart contracts with high transaction amounts (i.e., top 2000). In total, our reported SRVs affect a total amount of digital assets worth 428,600 USD.

==> figures/backup.tex <==
\begin{figure}[t]
\begin{lstlisting}
contract TokenisOwnable {
  function tokenAddresses() external { 
    address[] memory addresses = new address[](tokens.length);
    for (uint256 i = 0; i < tokens.length; i++) {
      addresses[i] = tokens.getAddress;}
    return addresses; }   
\end{lstlisting}

\caption{An example of false negative reported by baseline 2, which can be avoided by \system{} with the help of analyzing state R\&W relationship}
\label{CSexample}
%\vspace{-0.1in}
\end{figure}

==> figures/backupdos.tex <==
\begin{figure}[t]
\begin{lstlisting}
contract TokenGame {
  mapping(address => uint256) public SheepToken;
  mapping(address => uint256) public WolfToken;
  ...
  function MintToken(address account, unit amount) public{
    uint256 seed= (random () >> 245) % 10; 
    if ( seed != 0) {  
      SheepToken[account]++;} 
    else{
      WolfToken[account]++;}
    transferFrom (address(this), account, amount/2); }
  ...
}
    
contract Attacker {
  function onlyWolf(address target, bytes data) public{
    unit256 Before=WolfToken.balanceOf(address(this));
    target.call{value:0}(data);
    unit256 After=WolfToken.balanceOf(address(this));
    require(After > Before); 
    _transfer (address(this), msg.sender);}
}

\end{lstlisting}
\textbf{(a) Rollback.}
\begin{lstlisting}
contract Refunder {
  address[] private refundAddresses;
  mapping (address => uint) public refunds;
  function refundAll() public {
  for(uint x; x < refundAddresses.length; x++) { 
    require(refundAddresses[x].send(refunds[refundAddresses[x]])); }}}
\end{lstlisting}
\textbf{(b) DoS for unexpected Revert.}
\caption{The examples for illustrating Rollback and DoS for unexpected revert.}
\label{illustrateexample}
%\vspace{-0.1in}
\end{figure}

==> section432rename.tex <==
\subsubsection{xDFG construction based on data-flow reuse}
\label{subsec:xdfg}

%简单的思路是对于每一种漏洞，都需要构建CFG/DFG，但是这种方法很冗余，会导致额外的性能开销。因此对于跨合约我们提出重用DFG的概念，减小overhead。

\yuhong{By default, identifying each type of cross-contract vulnerabilities needs to individually run the complete data-flow analysis for all the involved contracts and functions. This would incur significant performance overhead, since cross-contract analysis typically involves longer call chains, in which the data-flow analysis is much more complex than the data-flow in a single contract. To further improve the efficiency of \system{}, a key observation here is that for analyzing different cross-contract vulnerabilities, the data-flow results for most functions in the call chain are exactly approximate regardless the vulnerabilities we aim to detect. 
%To illustrate, figure~\ref{fig:changeset} shows a concrete scenario regarding the different parts labeled by \system{} when analyzing timestamp manipulation (part (b)) after reentrancy (part (a)). As can be seen, the data-flow of nodes in green can be reused because they are not affected by the changed part (nodes in grey and yellow).
To this end, \system{} efficiently constructs the corresponding cross-contract data-flow graph (xDFG), by reusing part of the previously computed data-flow results. This process significantly eliminates the unnecessary (redundant) data-flow analysis without affecting the effectiveness for identifying different vulnerabilities.
}

Figure~\ref{fig:changeset} shows a concrete scenario regarding the different parts labeled by \system{} when analyzing timestamp manipulation (part (b)) after reentrancy (part (a)). As can be seen, the data-flow of nodes in green can be reused because they are not affected by the changed part (nodes in grey and yellow).

% \ZQ{
% In the cross-contract analysis, even though it is a significant performance overhead to compute the highly precise data-flow analysis on the extensive codes, but these analysis is still inefficient in the actual analysis process. A large margin of this inefficiency is due to the fact that the existing data-flow analysis used in smart contracts lacks a method to eliminate the redundant parts in the analysis process. For example, figure~\ref{fig:changeset} shows a concrete scenario regarding the different parts labeled by \system{} when analyzing timestamp manipulation (part (b)) after reentrancy (part (a)). As can be seen, data-flow of the nodes in green can be reused because they are not affected by the changed part (nodes in grey and yellow).
% Hence, during the inter-procedural analysis for identifying different vulnerabilities, \system{} efficiently constructs the corresponding cross-contract data-flow graph (xDFG), by reusing part of the previously computed data-flow results. This process significantly eliminates the unnecessary (redundant) data-flow analysis without affecting the effectiveness for identifying different vulnerabilities.
% }
\yuhong{We use Algorithm 1 to detail this data-flow reuse mechanism, which has the following three procedures.

\textbf{Procedure 1: identifying affected nodes}. To construct the new xDFG, \system{} needs to determine which part of data-flow results can be reused, by comparing the constructed xCFG for analyzing two different vulnerabilities. For ease of illustration, we call the xCFG used for analyzing the previous vulnerability as $xCFG_{prev}$, and the current xCFG as $xCFG_{curr}$. Then, \system{} identifies the changed part (as nodes $N_{c}$ and edges $E_{c}$) and the overlapped part based on an algorithm proposed in \cite{arzt2014reviser} which highlights the structural difference between the two xCFGs (line 1 in Algorithm-1). 

To this end, for the changed part, \system{} updates all the data-flow analysis results on these nodes; for the overlapped part, \system{} only needs to conduct the data-flow analysis on nodes affected by the changed part. To this end, all data-flow results of the rest nodes (denoted as safe nodes $N_{safe}$) can be reused because they are not affected by the difference between the two xCFGs. The affected nodes $N_{affected}$ are obtained by computing the reachability for all nodes in $N_{c}$ (line 2, 3 in Algorithm-1).  


\textbf{Procedure 2: safe data-flow propagation}. Once the affected nodes are computed, \system{} must make sure to perform a complete and precise data-flow repropagation among all the affected nodes $N_{affect}$. For the purpose of completeness and precision, the data-flow propagation generally starts from the safe nodes. Nonetheless, the optimal choice of start nodes ($N_{start}$) should be made for the data-flow repropagation, in order to avoid the unnecessary data-flow computation. Before we get to that, we give the definition of start node, for a given affected node $n_{affect}$ and a path $p$ to $n_{affect}$, a safe node $n_{safe}$ on this path is considered a start node if there is no other safe node closer to $n_{affect}$ on $p$. A key observation of this definition is that an affected node $n_{affect}$ can have multiple start nodes if there are multiple paths to $n_{affect}$. In this procedure, \system{} determine the start nodes $N_{start}$ through the following method. If the affected node $n_{affect}$ is inside a loop, the start node can be the safe node that is closest to the head of the loop $l_{s}$ (as illustrated in line 6, 7); if the affected node $n_{affect}$ is not in a loop, the start node should be the safe node that is closest to $n_{affect}$ (as illustrated in line 9).

\textbf{Procedure 3: cleaning and forward propagation}.
Once start nodes are known, a trivial approach would be to just pass over the changed program twice: One would first clear all outdated data-flow results at all affected nodes and then start a new propagation from each of the start nodes. For efficiency, however, \system{} follows a more advanced approach by combining both passes into a single clear-and-propagate step. When \system{} processes a node, it first clears the outdated results associated with this node to then compute the new analysis information through a propagation from the node's already re-computed predecessors. While efficient, this clear-and-propagate approach requires some precaution: if a node can be reached on more than one path, \system{} must make sure to clear it only once. In this procedure, \system{} use a clean list to remembers all nodes for which the analysis information has been cleared already, preventing them from being cleared a second time. In addition, while performing forward propagation, \system{} needs to guarantee itself to all reachable path from each affected node.  In this procedure, \system{} clean and forward propagate through the following method. First, \system{} divide the affected nodes into the merge node and normal node (as illustrated in line 10). For each merge node, \system{} should clean the outdated data-flow result while reaching it first, and perform the forward propagation after \system{} finish the computation of all its branches (as illustrated in line 12-15). For each normal node, \system{} performs the single clear-and-propagate step on it directly (as illustrated in line 17).  

}

\ZQ{
Next,this section explains the reused-based data-flow analysis algorithm used in \system{}, as illustrated in Algorithm 1. This algorithm can be generally divided into the following three procedures:

\textbf{Procedure 1: identifying affected nodes}. To construct the new xDFG, \system{} needs to determine which part of data-flow results can be reused by comparing the constructed xCFG for analyzing two different vulnerabilities. For ease of illustration, we call the xCFG used for analyzing the previous vulnerability as $xCFG_{p}$, and the current xCFG which tries to reuse the data-flow results of $xCFG_{prev}$ as $xCFG_{curr}$. \system{} first splits $xCFG_{prev}$ as two parts: namely, the changed part which $xCFG_{curr}$ does not contain, and the overlapped part which also exists in $xCFG_{curr}$. In our research, the changed part is denoted as the change nodes $N_{c}$ and edges $E_{c}$, calculated by an algorithm proposed in ~\cite{arzt2014reviser} which highlights the structural difference between the given two graphs (line 1 in Algorithm-1). For the changed part, \system{} needs to delete all the data-flow analysis results on these nodes. For the overlapped part, \system{} only needs to conduct the data-flow analysis on the nodes that are affected by the data-flow of the changed part. To this end, all data-flow results of the rest nodes (denoted as safe nodes $N_{safe}$) can be reused because they are not affected by the difference between the two xCFGs. In this procedure, the affected nodes $N_{affect}$ can be obtained by computing the reachability for all nodes in $N_{c}$ (line 2, 3 in Algorithm-1).  

\textbf{Procedure 2: safe data-flow propagation}. Once the affected nodes are computed, \system{} must make sure to perform a complete and precise data-flow repropagation among all the affected nodes $N_{affect}$. For the purpose of completeness and precision, the data-flow propagation generally starts from the safe nodes. Nonetheless, the optimal choice of start nodes (denoted as $N_{start}$) should be made for the data-flow repropagation, in order to avoid the unnecessary data-flow computation. Before we get to that, we give the definition of start node, for a given affected node $n_{affect}$ and a path $p$ to $n_{affect}$, a safe node $n_{safe}$ on this path is considered a start node if there is no other safe node closer to $n_{affect}$ on $p$. A key observation of this definition is that an affected node $n_{affect}$ can have multiple start nodes if there are multiple paths to $n_{affect}$. In this procedure, \system{} determine the start nodes $N_{start}$ through the following  method. If the affected node $n_{affect}$ is inside a loop, the start node can be the safe node that is closest to the head of the loop $l_{s}$ (as illustrated in line 6, 7); if the affected node $n_{affect}$ is not in a loop, the start node should be the safe node that is closest to $n_{affect}$ (as illustrated in line 9).


%在affectednodes被计算出来后，我们需要确保能在affectednodes中进行完整的数据流重传播计算。在本procedure中，我们将数据流可重用的节点称为safenode。为了确保smartdagger在affected nodes中数据流传播准确性和完整性，数据流传播的通常由safe nodes处开始。然而，为了避免safenode处不必要重计算，我们需要选择合适的数据流传播起点，用Nvertex表示。For a given affected node a and a path p to a, a safe node s on this path is considered a start node if there is no other safe node closer to s on p. 根据这个定义可以观察到，如果一个受影响的节点有多个(可传递的)前体，那么它们都是开始节点。在这个步骤中，我们确定传播起点的方法主要如下：对于在循环内的节点，那么距离循环起点ls处最近的safenode就是startnode；而对于不在循环内的节点，那么距离该节点最近的safenode就是startnode。

\textbf{Procedure 3: cleaning and forward propagation}.
Once start nodes are known, a trivial approach would be to just pass over the changed program twice: One would first clear all outdated data-flow results at all affected nodes and then start a new propagation from each of the start nodes. For efficiency, however, \system{} follows a more advanced approach by combining both passes into a single clear-and-propagate step. When \system{} processes a node, it first clears the outdated results associated with this node to then compute the new analysis information through a propagation from the node's already re-computed predecessors. While efficient, this clear-and-propagate approach requires some precaution: if a node can be reached on more than one
path, \system{} must make sure to clear it only once. In this procedure, \system{} use a clean list to remembers all nodes for which the analysis information has been cleared already, preventing them from being cleared a second time. In addition, while performing forward propagation, \system{} needs to guarantee itself to all reachable path from each affected node.  In this procedure, \system{} clean and forward propagate through the following method. First, \system{} divide the affected nodes into the merge node and normal node (as illustrated in line 10). For each merge node, \system{} should clean the outdated data-flow result while reaching it first, and perform the forward propagation after \system{} finish the computation of all its branches (as illustrated in line 12-15). For each normal node, \system{} performs the single clear-and-propagate step on it directly (as illustrated in line 17).  
}
%To construct the new xDFG, \system{} needs to determine which part of data-flow results can be reused by comparing the constructed xCFG for analyzing two different vulnerabilities. For ease of illustration, we call the xCFG used for analyzing the previous vulnerability as $xCFG_{p}$, and the current xCFG which tries to reuse the data-flow results of $xCFG_{prev}$ as $xCFG_{curr}$. \system{} first splits $xCFG_{prev}$ as two parts: namely, the changed part which $xCFG_{curr}$ does not contain, and the overlapped part which also exists in $xCFG_{curr}$. In our research, the changed part is calculated based on an algorithm proposed in ~\cite{arzt2014reviser} which highlights the structural difference between the given two graphs. For the changed part, \system{} needs to delete all the data-flow analysis results on these nodes. For the overlapped part, \system{} only needs to conduct the data-flow analysis on the nodes that are affected by the data-flow of the changed part. To this end, all the rest data-flow results can be reused because they are not affected by the difference between the two xCFGs.



\begin{table}[htb]\small\addtolength{\tabcolsep}{-3pt}
	%\caption{Parameter Configuration.}
	\normalsize % Font size can be changed to match table content. Recommend 10 pt.
	%\centering
\vspace{0.1in}
\ZQ{
	\begin{tabular}{ l }

		\hline\noalign{\smallskip}
		\textbf{Algorithm 1:} Reused-based data-flow analysis\\
		\noalign{\smallskip}\hline\noalign{\smallskip}
		%\textbf{Input}: $C_a$, $C_{th}$, $C_m$, $G$, $L_m$, $R$, $P_{as}$, $N1$;                               \\
		%\textbf{Output}: $t$,$l$;            \\
        \textbf{Procedure 1}: identifying affected node ($xCFG_{prev},xCFG_{curr}$) \\
		1: \ \ \ \   $<E_{c},N_{c}> := ComputexCFGchanges
		(xCFG_{prev},xCFG_{curr}$) \\
		2: \ \ \ \  \textbf{for} all $n \in N_{c}$ \textbf{do}\\
		3: \ \ \ \ \ \ \ \ $N_{affect} := ComputeReachability(n)$ \\ 
		\textbf{Procedure 2}: safe data-flow propagation ($N_{affect}$) \\
		4: \ \ \ \  \textbf{for} all $(n_{1},n_{2}) \in N_{affect}$ \textbf{do} \\
		5: \ \ \ \ \ \ \ \ \textbf{if} InsideLoop($n_{1}$) \textbf{then} \\
		6: \ \ \ \ \ \ \ \ \ \ \ \ $l_{s} := ComputeLoopStart (n_{1})$ \\
		7: \ \ \ \ \ \ \ \ \ \ \ \ $N_{start} := GetPredsOf(l_{s})$ \\
		8: \ \ \ \ \ \ \ \ \textbf{else} \\
		9: \ \ \ \ \ \ \ \ \ \ \ \ $N_{start} := GetPredsOf(n_{1})$ \\
		\textbf{Procedure 3}: cleaning and forward propagation ($N_{affect}, N_{start}$) \\
		10: \ \ \ \ $N_{merge} := GetMergePoint(N_{affect})$ \\
		11: \ \ \ \  \textbf{for} all $n \in N_{affect}$ \textbf{do}\\
		12: \ \ \ \ \ \ \ \ \textbf{if} $n \in N_{merge}; CheckCleanList; !Checkbranch$ \textbf{then} \\
		13: \ \ \ \ \ \ \ \ \ \ \ \ $Clean(n)$ \\
		14: \ \ \ \ \ \ \ \ \textbf{else if} $n \in N_{merge}; !CheckCleanList;  Checkbranch$ \\
		15: \ \ \ \ \ \ \ \ \ \ \ \ $ForwardPropagate(n)$ \\
		16: \ \ \ \ \ \ \ \ \textbf{else} \\
		17: \ \ \ \ \ \ \ \ \ \ \ \ $CleanandForwardPropagate(n)$ \\
		\hline
	\end{tabular} 
	
}
\label{algorithm1}
\end{table}


%To this end, the data-flow propagate analysis can be divided into three steps. (1) \system{} clears the previous analysis results on these affected nodes. (2) \system{} computes the predecessors for each affected node, and finds the affected nodes without predecessors, which are regarded as the vertexes of the affected set. Finally, \system{} starts from the vertexes and performs the forward-only data-flow analysis on the affected nodes. 
 
 %identify affected nodes （）
 
 %re-propagations
 
 %function call
 

 


==> tables/evaluation-baselineP.tex <==
\begin{table}[b]
%\vspace{0.3in}
\caption{Precision rate for graph construction experiment on Ethereum open dataset.}

\begin{tabular}{l|ccc|ccc}
\hline
Approach                                                     & \multicolumn{3}{c|}{Baseline 2}                                              & \multicolumn{3}{c}{\system{}}                                                  \\ \hline
                                                                  & \multicolumn{1}{l}{TP} & \multicolumn{1}{l}{FP} & \multicolumn{1}{l|}{prec.} & \multicolumn{1}{l}{TP} & \multicolumn{1}{l}{FP} & \multicolumn{1}{l}{prec.} \\ \hline
Rollback                                                          & 35                     & 20                     & 63.64\%                    & 77                     & 12                      & 86.52\%                   \\
\begin{tabular}[c]{@{}l@{}}Dos (unexpected\\ Revert)\end{tabular} & 245                    & 201                    & 54.93\%                    & 574                    & 108                     & 84.16\%                   \\ \hline
Total                                                             & 280                    & 221                    & 55.89\%                    & 651                    & 120                     & 84.44\%                   \\ \hline
\end{tabular}
\label{table:graphconstruction}
\end{table}

==> tables/evaluation-efficiency.tex <==
\begin{table}[hptb]
\vspace{0.3in}
\caption{Efficiency experiment.}

\begin{tabular}{l|cc|cc}
\hline
                                                                  & \multicolumn{2}{c|}{Ethereum dataset}                         & \multicolumn{2}{c}{Annotated dataset}                         \\ \hline
Vulnerability                                                     & \multicolumn{1}{l}{Avg.time (s)} & \multicolumn{1}{l|}{prec.} & \multicolumn{1}{l}{Avg.time (s)} & \multicolumn{1}{l}{recall} \\ \hline
Rollback                                                          &                                  &                            &                                  &                            \\
\begin{tabular}[c]{@{}l@{}}Dos (unexpected\\ Revert)\end{tabular} &                                  &                            &                                  &                            \\ \hline
Total                                                             &                                  &                            &                                  &                            \\ \hline
\end{tabular}

\label{semantic}
\end{table}

==> tables/evaluation-precision.tex <==

\begin{table*}[h]
\vspace{0.3in}

\caption{Overall precision for different tools on the evaluation dataset.}

\begin{tabular}{l|ccc|ccc|ccc|ccc}
\hline
Vulnerability                                                     & \multicolumn{3}{l|}{eTainer}                                                 & \multicolumn{3}{l|}{Slither}                                                 & \multicolumn{3}{l|}{Madmax}                                                  & \multicolumn{3}{l}{system}                               \\ \hline
                                                                  & \multicolumn{1}{l}{TP} & \multicolumn{1}{l}{FP} & \multicolumn{1}{l|}{prec.} & \multicolumn{1}{l}{TP} & \multicolumn{1}{l}{FP} & \multicolumn{1}{l|}{prec.} & \multicolumn{1}{l}{TP} & \multicolumn{1}{l}{FP} & \multicolumn{1}{l|}{prec.} & TP  & \multicolumn{1}{l}{FP} & \multicolumn{1}{l}{prec.} \\ \hline
Rollback                                                          & -                      & -                      & -                          & -                      & -                      & -                          & -                      & -                      & -                          & 77  & 12                     & 86.52\%                   \\
\begin{tabular}[c]{@{}l@{}}Dos (unexpected\\ Revert)\end{tabular} & 178                    & 215                    & 45.29\%                    & 181                    & 2555                   & 7.08\%                     & 19                     & 54                     & 26.03\%                    & 574 & 108                    & 84.16\%                   \\ \hline
Total                                                             & 178                    & 215                    & 45.29\%                    & 181                    & 2555                   & 7.08\%                     & 19                     & 54                     & 26.03\%                    & 651 & 120                    & 84.44\%                   \\ \hline
\end{tabular}
\tabnote{\\ “-” means the corresponding tool does not support detecting this type of vulnerability.}

\label{tableprec.ision}
\end{table*}


==> tables/evaluation-recall.tex <==
\begin{table*}[h]
\vspace{0in}

\caption{Overall recall rate for different tools on the tool evaluation dataset.}
\begin{tabular}{l|ccc|ccc|ccc|ccc}
\hline
Vulnerability                                                     & \multicolumn{3}{c|}{eTainer}                                                  & \multicolumn{3}{c|}{Slither}                                                  & \multicolumn{3}{c|}{Madmax}                                                   & \multicolumn{3}{c}{system}                                                    \\ \hline
                                                                  & \multicolumn{1}{l}{TN} & \multicolumn{1}{l}{FN} & \multicolumn{1}{l|}{recall} & \multicolumn{1}{l}{TN} & \multicolumn{1}{l}{FN} & \multicolumn{1}{l|}{recall} & \multicolumn{1}{l}{TN} & \multicolumn{1}{l}{FN} & \multicolumn{1}{l|}{recall} & \multicolumn{1}{l}{TN} & \multicolumn{1}{l}{FN} & \multicolumn{1}{l}{recall.} \\ \hline
Rollback                                                          & -                      & -                      & -                           & -                      & -                      & -                           & -                      & -                      & -                           & 23                     & 4                      & 85.19\%                     \\
\begin{tabular}[c]{@{}l@{}}Dos (unexpected\\ Revert)\end{tabular} & 25                     & 39                     & 39.06\%                     &21                        &43                        &32.81\%                             & 11                     & 53                     & 17.19\%                     & 58                     & 6                      & 90.63\%                     \\ \hline
Total                                                             & 25                     & 39                     & 39.06\%                     &21                        &43                        & 32.81\%                            & 11                     & 53                     & 17.19\%                     & 81                     & 10                     & 89.01\%                     \\ \hline
\end{tabular}
\tabnote{\\ “-” means the corresponding tool does not support detecting this type of vulnerability.}

\label{recall}
\end{table*}

==> tables/meth-filtering.tex <==
\begin{table}[b]
\scriptsize
\caption{Function selection rules for locating different vulnerability}
\begin{tabular}{|l|c|}
\hline
Vulnerability type               & Function selection rule                                                                                                           \\ \hline
R1-Reentrancy             & \begin{tabular}[c]{@{}c@{}}$\left( isContained (external call) \wedge isModified (Banlance) \right)  \vee$ \\ $ isModified (var_{state})$ \end{tabular}                                                                      \\ \hline
R2-Taint for owner             & \begin{tabular}[c]{@{}c@{}}$(isModified (Owner) \wedge isAuthorized (owner)) \vee $ \\ $isModified (var_{state})$\end{tabular} \\ \hline
R3-Timestamp manipulation              &   \begin{tabular}[c]{@{}c@{}}$isExectionLock (Timestamp) \vee isModified (var_{state})$ \end{tabular}                                                                                                                            \\ \hline
R4-Dos attack             & $isChecked (External call) \vee isModified (var_{state})$                                                                                                                              \\ \hline
\end{tabular}
\label{table-filtering}
\end{table}

==> tables/motivatingexample.tex <==
\begin{figure}[t]
\begin{lstlisting}
contract Barn {
  function claimFromBarn(tokenId, unstake) external {
    if (isSheep(tokenId)){
      owed=_claimSheepFromBarn(tokenId, unstake);}
      WOOL._mint(msg.sender, owed);}
  
  function _claimSheepFromBarn(tokenId, unstake) internal return (owed){
    unit256 owed = 10000;  //ERC20 Token $WOOL
    if (unstake) {
      // 50% chance of all $WOOL stolen, punishment
      if (random(tokenId) & 1 == 1) { 
        _payWolfTax(owed);
        owed = 0;}
    else {
      // 20% tax to pay
      _payWolfTax(owed * 20 / 100);}}}
}

contract Attacker {
  function FreeofTax(Barn target, tokenId) public{
    target.claimFromBarn(tokenId, True);
    unit256 After = WOOL.balanceOf(address(this));
    require(After == 10000); }
}

\end{lstlisting}
\end{figure}
